The AeroSonicDB (YPAD-0523) Dataset for Acoustic Detection and Classification of Aircraft

The time and expense required to collect and label audio data has been a prohibitive factor in the availability of domain specific audio datasets. As the predictive specificity of a classifier depends on the specificity of the labels it is trained on, it follows that finely-labelled datasets are crucial for advances in machine learning. Aiming to stimulate progress in the field of machine listening, this paper introduces AeroSonicDB (YPAD-0523), a dataset of low-flying aircraft sounds for training acoustic detection and classification systems. This paper describes the method of exploiting ADS-B radio transmissions to passively collect and label audio samples. Provides a summary of the collated dataset. Presents baseline results from three binary classification models, then discusses the limitations of the current dataset and its future potential. The dataset contains 625 aircraft recordings ranging in event duration from 18 to 60 seconds, for a total of 8.87 hours of aircraft audio. These 625 samples feature 301 unique aircraft, each of which are supplied with 14 supplementary (non-acoustic) labels to describe the aircraft. The dataset also contains 3.52 hours of ambient background audio ("silence"), as a means to distinguish aircraft noise from other local environmental noises. Additionally, 6 hours of urban soundscape recordings (with aircraft annotations) are included as an ancillary method for evaluating model performance, and to provide a testing ground for real-time applications.

==> location_distribution.tex <==
\begin{table}[H]
\centering
\begin{tabular}{lrrrr}
    \toprule
    \textbf{location} &     0 &   1 &    2 &  TOTAL \\
    \textbf{class} &       &     &      &        \\
    \midrule
    \textbf{0    } &  27.1 &  0.3 &   1.0 &   28.4 \\
    \textbf{1    } &  69.9 &  0.6 &   1.2 &   71.6 \\
    \midrule
    \textbf{TOTAL} &  97.0 &  0.9 &  2.2 &   100.0 \\
    \bottomrule
\end{tabular}
\caption{Distribution of samples by location (\%).}
\end{table}

==> metrics-table.tex <==
\begin{tabular}{lrr}
\toprule
Model &   Mean Accuracy &   Std. Dev. \\
\midrule
Logistic Regression    & 93.66 & 3.86 \\
MLP    & 94.74 & 4.67 \\
CNN   & 93.83 & 4.52 \\
RNN-LSTM    & 93.13 & 8.40 \\
\bottomrule
\end{tabular}

==> microphone_distribution.tex <==
\begin{table}[H]
\centering
\begin{tabular}{lrrr}
    \toprule
    \textbf{microphone} &     0 &     1 &  TOTAL \\
    \textbf{class} &       &       &        \\
    \midrule
    \textbf{0            } &   3.9 &   24.5 &    28.4 \\
    \textbf{1            } &  11.9 &  59.8 &   71.6 \\
    \midrule
    \textbf{TOTAL        } &  15.8 &  84.2 &   100.0 \\
    \bottomrule
\end{tabular}
\caption{Distribution of samples by microphone (\%).}
\end{table}
